Literature-Grounded Novelty Assessment of Scientific Ideas

Automated scientific idea generation systems have made remarkable progress, yet the automatic evaluation of idea novelty remains a critical and underexplored challenge. Manual evaluation of novelty through literature review is labor-intensive, prone to error due to subjectivity, and impractical at scale. To address these issues, we propose the Idea Novelty Checker, an LLM-based retrieval-augmented generation (RAG) framework that leverages a two-stage retrieve-then-rerank approach. The Idea Novelty Checker first collects a broad set of relevant papers using keyword and snippet-based retrieval, then refines this collection through embedding-based filtering followed by facet-based LLM re-ranking. It incorporates expert-labeled examples to guide the system in comparing papers for novelty evaluation and in generating literature-grounded reasoning. Our extensive experiments demonstrate that our novelty checker achieves approximately 13% higher agreement than existing approaches. Ablation studies further showcases the importance of the facet-based re-ranker in identifying the most relevant literature for novelty evaluation.

==> backup.tex <==













 




==> paper/limitations.tex <==
\section{Limitations and Future Work}


Our approach has several key limitations. First, due to context size constraints (since we include roughly fifteen in-context examples for both the novel and not novel categories), we restrict our analysis to the top 10 retrieved papers. This limitation may constrain the evaluation by making the selection of these top 10 papers disproportionately influential in determining the overall novelty. Second, our definition of novelty relies on expert annotations; should the definition change, this reannotation process can be both costly and time-consuming. Lastly, while our current retrieval strategy is effective, future work will potentially expand the scope of literature considered for novelty evaluation similar to \href{https://openai.com/index/introducing-deep-research/}{Deep Research} style literature search or using tools like ScholarQA \cite{singh_ai2_2025}to compare the input idea against a broader range of literature.









